Lower bounds on the size of semidefinite programming relaxations

We introduce a method for proving lower bounds on the efficacy of semidefinite programming (SDP) relaxations for combinatorial problems. In particular, we show that the cut, TSP, and stable set polytopes on $n$-vertex graphs are not the linear image of the feasible region of any SDP (i.e., any spectrahedron) of dimension less than $2^{n^c}$, for some constant $c > 0$. This result yields the first super-polynomial lower bounds on the semidefinite extension complexity of any explicit family of polytopes. Our results follow from a general technique for proving lower bounds on the positive semidefinite rank of a matrix. To this end, we establish a close connection between arbitrary SDPs and those arising from the sum-of-squares SDP hierarchy. For approximating maximum constraint satisfaction problems, we prove that SDPs of polynomial-size are equivalent in power to those arising from degree-$O(1)$ sum-of-squares relaxations. This result implies, for instance, that no family of polynomial-size SDP relaxations can achieve better than a 7/8-approximation for MAX-3-SAT.

==> content/introduction.tex <==

\section{Introduction}

Convex characterizations and relaxations of combinatorial problems has been
a consistent, powerful theme in the theory of algorithms since its inception.
Linear and semidefinite programming relaxations have been particularly useful
for the efficient computation of approximate solutions to NP-hard problems (see,
for instance, the books \cite{WS11,VaziraniBook01}).
In some sense, semidefinite programs (SDPs) can be seen as combining
the rich expressiveness of linear programs with the global geometric power of spectral methods.
For many fundamental combinatorial problems, this provides a genuinely new
structural and computational perspective \cite{GW95,KMS98,ARV09}.
Indeed, for an array of optimization problems, the best-known approximation algorithms can
only be achieved via SDP relaxations.

It has long been known that integrality gaps for linear programs (LPs) can often
lead to gadgets for NP-hardness of approximation reductions (see, e.g., \cite{DBLP:conf/stoc/LundY93,kcenter05,HK03}).
Furthermore, assuming the Unique Games Conjecture \cite{DBLP:conf/stoc/Khot02a},
it is known that integrality gaps for SDPs can
be translated directly into hardness of approximation results \cite{DBLP:conf/focs/KhotKMO04,Austrin10,Raghavendra08}.
All of this suggests that the computational model underlying LPs and SDPs is remarkably powerful.

Thus it is a natural (albeit ambitious) goal to
characterize the computational power of this model.  If $\mathrm{P} \neq \mathrm{NP}$, we do not expect
to find polynomial-size families of SDPs that yield arbitrarily good approximations
to NP-hard problems.  (See \cite{Rothvoss2013,DBLP:conf/esa/BrietDP13} for a discussion
of how this follows formally from the assumption $\mathrm{NP} \nsubseteq \mathrm{P}/\mathrm{poly}$.)


In the setting of linear programs (LPs), the search for a model and characterization
began in a remarkable work of Yannakakis \cite{Yannakakis91}.
He proved that the TSP and matching polytopes do not admit \emph{symmetric} linear programming
formulations of size $2^{o(n)}$, where $n$ is the number of vertices
in the underlying graph.  In the process, he laid the structural framework (in terms
of nonnegative factorizations) that would underlie all future work in the subject.
It took over 20 years before Fiorini, Massar, Pokutta, Tiwary, and de Wolf \cite{FMPTW12}
were able to remove the symmetry assumption and obtain a lower bound of $2^{\Omega(\sqrt{n})}$ on the
size of any LP formulation.  Soon afterward, Rothvo\ss\ \cite{DBLP:conf/stoc/Rothvoss14}
gave a lower bound of $2^{\Omega(n)}$ on the size of any LP formulation for the matching polytope
(and also TSP), completing Yannakakis' vision.

\Dnote{}

\Jnote{}

Despite the progress in understanding the power of LP formulations,
it remained a mystery whether there were similar strong lower bounds in the setting of SDPs.
An analogous positive semidefinite factorization framework
was provided in \cite{FMPTW12,GouveiaParriloThomas2011}.
Following the LP methods of \cite{DBLP:conf/focs/ChanLRS13},
the papers  \cite{DBLP:conf/coco/LeeRST14,FSP14} proved
exponential
lower bounds  on the size of \emph{symmetric} SDP formulations for NP-hard constraint satisfaction problems (CSPs).

In the present work, we prove strong lower bounds
on the size of general SDP formulations for the cut, TSP, and stable set polytopes.
Moreover, we show that polynomial-size SDP relaxations cannot achieve
arbitrarily good approximations for many NP-hard constraint satisfaction problems.
For instance, no polynomial-size family of relaxations
can achieve better than a $7/8$-approximation for \maxthreesat.  More
generally, we show that the low-degree sum-of-squares SDP
relaxations yield the best approximation among all polynomial-sized
families of relaxations for max-CSPs.

This is achieved by relating arbitrary SDP formulations to those coming from
the sum-of-squares SDP hierarchy\footnote{This hierarchy
is also frequently referred to as the Lasserre SDP hierarchy.} \cite{Lasserre01,Parrilo00,Shor87}, analogous to
our previous work with Chan relating LP formulations to the Sherali--Adams hierarchy \cite{DBLP:conf/focs/ChanLRS13}.
The SDP setting poses a number of significant challenges.
At a very high level, our approach can be summarized as follows:  Given an arbitrary SDP formulation
of small size, we use methods from quantum entropy maximization and online convex optimization (often going by
the name ``matrix multiplicative weights update'') to \emph{learn} an approximate low-degree sum-of-squares
formulation on a subset of the input variables.
In the next section, we present a formal overview of our results, and a discussion
of the connections to quantum information theory, real algebraic geometry, and proof complexity.

\paragraph{Organization}  The results of this work fall along two
broad themes, lower bounds on spectrahedral lifts of specific
polytopes and lower bounds on SDP relaxations for constraint
satisfaction problems.
Both sets of results are consequences
of a general method for proving lower bounds
on positive semidefinite rank.
For the convenience of the reader, we have
organized the two themes in two self-contained trajectories.  Thus, lower
bounds on spectrahedral lifts can be accessed via
\pref{sec:spectr-lifts-polyt}, \pref{sec:sos-degree},
\pref{sec:proofoverview}, \pref{sec:theproof} and
\pref{sec:corr}.  The lower bounds for constraint
satisfaction problems can be reached through \pref{sec:optimization},
\pref{sec:sos-degree}, \pref{sec:proofoverview},
\pref{sec:theproof} and \pref{sec:maxcsp}.

We also present general results on approximating density operators
against families of linear tests through quantum learning in
\pref{sec:learning}.  Finally, in \pref{sec:nnr}, we exhibit applications of our
techniques to non-negative rank; in particular, this is used
to give a simple, self-contained proof of a lower bound on the nonnegative rank of the unique disjointness
matrix.

\Pnote{}

\subsection{Spectrahedral lifts of polytopes}
\label{sec:spectr-lifts-polyt}
Polytopes are an appealing and useful way to encode many combinatorial optimization problems.
For example, the traveling salesman problem on $n$ cities is equivalent to optimizing linear functions over the traveling salesman polytope, i.e., the convex hull of characteristic vectors $\Ind_{C}\in \{0,1\}^{\binom n 2} \subseteq \mathbb R^{\binom n 2}$ of $n$-vertex Hamiltonian cycles $C$ (viewed as edge sets).
If a polytope admits polynomial-size LP or SDP formulations, then we can optimize linear functions over the polytope in polynomial time (exactly for LP formulations and up to arbitrary accuracy in the case of SDP formulations).
Indeed, a large number of efficient, exact algorithms for combinatorial
optimization problems can be explained by small LP or SDP formulations of the underlying polytope.
(For approximation algorithms, the characterization in terms of compact formulations of polytopes is not as direct \cite{DBLP:conf/focs/BraunFPS12}.
In \pref{sec:semid-relax-constr}, we will give a direct characterization for approximation algorithms in terms of the original combinatorial problem.)
%
%
%
%
%
%
%
%
%
%

\Dnote{}

\paragraph{Positive semidefinite lifts}
Fix a polytope $P \subseteq \mathbb R^n$ (e.g., the traveling salesman polytope described above).
We are interested in the question of whether there exists a low-dimensional SDP that captures $P$.
Let $\cS_+^k$ denote
the cone of symmetric, $k \times k$ positive semidefinite matrices embedded
naturally in $\mathbb R^{k \times k}$.  If there exists
an affine subspace $\cL \subseteq \mathbb R^{k \times k}$ and a linear
map $\pi : \mathbb R^{k \times k} \to \mathbb R^n$ such
that
\[
P = \pi(\cS_+^k \cap \cL)\,,
\]
one says that $P$ admits a \emph{positive-semidefinite (psd) lift of size $k$.} (This terminology is taken from \cite{FGPRT14}.)
We remark that the intersection of a PSD cone with an affine subspace
is often referred to as a \emph{spectrahedron.}

The point is that in order to optimize a linear function $\ell\from \R^n\to \R$ over the polytope $P$, it is enough to optimize the linear function $\ell\circ \pi\from \R^{k\times k}\to \R$ over the set $\cS^k_+ \cap \cL$ instead,
%
%
\begin{equation*}\label{eq:sdp-opt}
%
\min_{x \in P}\, \ell(x) = \min_{y \in \cS_+^k \cap \cL}  \ell\circ \pi (y)\mper
\end{equation*}
Here, the optimization problem on the right is a semidefinite programming problem in $k$-by-$k$ matrices.
This idea also goes under the name of a \emph{semidefinite extended formulation} \cite{FMPTW12}.

\Dnote{}

\paragraph{The positive-semidefinite rank of explicit polytopes}
We define the \emph{positive-semidefinite (psd) rank} of a polytope $P$, denoted $\psdrank(P)$, to be the smallest number $k$ such that there exists a psd lift of size $k$.
(Our use of the word ``rank'' will make sense soon---see \pref{sec:sos-degree}.)
Bri\"et, Dadush, and Pokutta
\cite{DBLP:conf/esa/BrietDP13}
showed (via a counting argument)
that there exist 0/1 polytopes in $\R^n$ with exponential psd rank.
 %
%
%
In this work, we prove the first super-polynomial lower bounds on the psd rank of explicit polytopes:
The correlation polytope  $\corr_n \subseteq \mathbb R^{n^2}$ is given by
\[
\corr_n = \mathrm{conv}\left(\{ xx^T : x \in \{0,1\}^n \}\right).
\]
In \pref{sec:psd-corr}, we show the following strong lower bound on its psd rank.
%
%
\begin{theorem}\label{thm:corr-lb}
For every $n \geq 1$, we have
\[
\psdrank(\corr_n) \geq 2^{\Omega(n^{2/13})}\,.
\]
\end{theorem}

The importance of the correlation polytope $\corr_n$ lies in the fact that
a number of interesting polytopes from combinatorial optimization contain
a face that linearly projects to $\corr_n$ .  We first define a few different families
of polytopes and then recall their relation to $\corr_n$.

For $n \geq 1$,
let $K_n = ([n], {[n] \choose 2})$ be the complete graph on $n$ vertices.
For a set $S \subseteq [n]$, we use $\partial S \subseteq {[n] \choose 2}$ to denote the set of edges
with one endpoint in $S$ and the other in $\bar S$, and we use the notation $\1_{\partial S} \in \mathbb R^{n \choose 2}$
to denote the characteristic vector of $S$.  The \emph{cut polytope on $n$ vertices} is defined by
\[
\cut_n = \mathrm{conv} \left(\{ \1_{\partial S} : S \subseteq [n] \} \right).
\]
Similarly, if $\tau$ is a salesman tour of $K_n$ (i.e., a Hamiltonian cycle), we use $\1_{E(\tau)} \in \mathbb R^{n \choose 2}$ to
denote the corresponding indicator of the edges contained in $\tau$.  In that case, the \emph{TSP polytope} is given by
\[
\tsp_n = \mathrm{conv} \left(\{ \1_{E(\tau)} : \text{ $\tau$ is a Hamiltonian cycle} \} \right).
\]
Finally, consider an arbitrary $n$-vertex graph $G=([n], E)$.  We recall that a subset of vertices $S \subseteq [n]$
is an \emph{independent set} (also called a stable set) if there are no edges between vertices in $S$.  The \emph{stable set
polytope of $G$} is given by
\[
\stab_n(G) = \mathrm{conv} \left( \{\1_S \in \mathbb R^{n} : S \textrm{ is an independent set in $G$}\}\right).
\]
By results of \cite{DeSimone90} and \cite{FMPTW12} (see \pref{prop:polytope-relations}), \pref{thm:corr-lb} directly implies the following lower bounds on the  psd rank of the cut, TSP, and stable set polytopes.
\begin{corollary}
The following lower bounds hold for every $n \geq 1$,
\begin{align*}
& \psdrank(\cut_n) \geq 2^{\Omega(n^{2/13})}, \\
& \psdrank(\tsp_n) \geq 2^{\Omega(n^{1/13})}, \\
\max_{\textrm{$n$-vertex $G$}} & \psdrank(\stab_n(G))  \geq 2^{\Omega(n^{1/13})}.
\end{align*}
\end{corollary}


\subsection{Semidefinite relaxations and constraint satisfaction}
\label{sec:optimization}
\label{sec:semid-relax-constr}
%
%
%
%
We now formalize a computational model of semidefinite relaxations for combinatorial optimization problems and prove strong lower bounds for it.
Unlike the polytope setting in the previous section, this model also allows us to capture approximation algorithms directly.
\Dnote{}

%
%
Consider the following general optimization problem:%
\footnote{In this section, we restrict our discussion to optimization problems over the discrete cube.
Some of our results also apply to other problems, e.g., the traveling salesman problem (albeit only for exact algorithms).}
Given a low-degree function $f\from \{0,1\}^n\to \R$, represented by its coefficients as a multilinear polynomial,
\begin{equation}
\label{eq:hypercube-optimization}
  \begin{gathered}
    \text{maximize }f(x)\\
    \text{subject to } x\in \{0,1\}^n\mper
  \end{gathered}
\end{equation}
Many basic optimization problems are special cases of this general problem, corresponding to functions $f$ of a particular form:
For the problem of finding the maximum cut in a graph $G$ with $n$ vertices, the function $f$ outputs on input $x\in \{0,1\}^n$ the number of edges in $G$ that cross the bipartition represented by $x$, i.e., $f(x)$ is the number of  edges $\{i,j\}\in E(G)$ with $x_i\neq x_j$.
Similarly, for \maxthreesat on a 3CNF formula $\varphi$ with $n$ variables, $f(x)$ is the number of clauses in $\varphi$ satisfied by the assignment $x$.
More generally, for any $k$-ary boolean constraint satisfaction problem, the function $f$ counts the number of satisfied constraints.
Note that in these examples, the functions have at most degree $2$, degree $3$, and degree $k$, respectively.

Algorithms with provable guarantees for these kinds of problems---either implicitly or explicitly---certify upper bounds on the optimal value of instances.
(Indeed, for solving the decision version of these optimization problems, it is enough to provide such certificates.)
It turns out that the best-known algorithms for these problems are captured by certificates of a particularly simple form, namely sums of squares of low-degree polynomials.
The following upper bounds on problems of the form \pref{eq:hypercube-optimization} are equivalent to the relaxations obtained by the sum-of-squares SDP hierarchy \cite{Lasserre01,Parrilo00,Shor87}.
For $f : \{0,1\}^n \to \R$, we use $\deg(f)$ to denote the degree of the unique
multilinear real polynomial agreeing with $f$ on $\{0,1\}^n$; see \pref{sec:prelims}.

\newcommand{\sosub}{\overline{\textup{sos}}}


\Jnote{}

\begin{definition}
  The \emph{degree-$d$ sum-of-squares upper bound} for a function $f \from \{0,1\}^n\to \R$, denoted $\sosub_d(f)$, is the smallest number $c\in \R$ such that $c-f$ is a sum of squares of functions of degree at most $d/2$, i.e., there exists functions $g_1,\ldots,g_t\from \{0,1\}^n\to \R$ for some $t\in \N$ with $\deg(g_1),\ldots,\deg(g_t)\le d/2$ such that the following identity between functions on the discrete cube holds:
  \begin{displaymath}
    c- f = g_1^2 + \cdots g_t ^2\mper
  \end{displaymath}
\end{definition}
Every function $f$ satisfies $\sosub_d(f)\ge \max (f)$ since sums of squares of real-valued functions are nonnegative pointwise.
For $d \geq 1$,
the problem of computing $\sosub_d(f)$ for a given function $f\from \{0,1\}^n\to \R$ (of degree at most $d$) is a semidefinite program of size
at most $1+ n^{d/2}$ (see, e.g., Theorem \ref{thm:gtwo-pseudodist}).%
\footnote{Moreover, for every $d\in \N$, there exists an $n^{O(d)}$-time algorithm based on the ellipsoid method that, given $f$, $c$, and $\e>0$, distinguishes between the cases $\sosub_d(f)\ge c$ and $\sosub_d(f)\le c-\e$ (assuming the binary encoding of  $f$, $c$, and $\e$ is bounded by $n^{O(d)}$).}
%

The $\sosub_d$ upper bound is equivalent to the degree-$d$
sum-of-squares (also known as the level-$d/2$ Lasserre) SDP bound, and for small values
of $d$, these upper bounds underlie the best-known approximation algorithms for several
optimization problems.
For example, the Goemans--Williamson algorithm for \maxcut is based on the upper bound $\sosub_2$.
If we let $\alpha_{GW}\approx 0.878$ be the approximation ratio of
this algorithm, then every graph $G$ satisfies $\max (f_G) \ge
\alpha_{GW}\cdot \sosub_2(f_G)$ where the function $f_G$ measures cuts in $G$, i.e., $f_G(x)\coloneq \sum_{ij\in E(G)}(x_i-x_j)^2$.


A natural generalization of low-degree sum-of-squares certificates is
obtained by summing squares of functions in a low-dimensional
subspace.  We can formulate this generalization as a {\it non-uniform}
model of computation that captures general semidefinite programming
relaxations.  First, we make the following definition for a subspace
of functions.

\begin{definition}
\label{def:subspace-u-sos-ub}
  For a subspace $U$ of real-valued functions on $\{0,1\}^n$, the \emph{subspace-$U$ sum-of-squares upper bound} for a function $f\from \{0,1\}^n\to \R$, denoted $\sosub_U(f)$, is the smallest number $c\in \R$ such that $c-f$ is a sum of squares of functions from $U$, i.e., there exist a $g_1,\ldots,g_t\in U$ such that $c-f=g_1^2+\cdots + g_t^2$ is an identity of functions on $\{0,1\}^n$.
\end{definition}

Here, the subspace $U$ can be thought of as ``non-uniform advice'' to an
algorithm, where its dimension $\dim(U)$ is the size of advice.
%
In fact, if we fix this advice $U$, the problem of computing $\sosub_U(f)$ for a given function $f$ has a semidefinite programming formulation of size $\dim(U)$.%
\footnote{Under mild conditions on the subspace $U$, there exists a boolean circuit of size $(\dim U)^{O(1)}$ that given a constant-degree function $f$, and number $c\in \R$ and $\e>0$, distinguishes between the cases $\sosub_U(f)\ge c$ and $\sosub_U(f)\le c-\e$ (assuming the bit encoding length of $f$, $c$, and $\e$ is bounded by $(\dim U)^{O(1)}$.).
Note that since we will prove lower bounds against this model, the possibility that some subspaces might not correspond to small circuits does not weaken our results.
}
%
Moreover, it turns out that the generalization captures, in a certain precise
sense, all possible semidefinite programming relaxations for
\pref{eq:hypercube-optimization}.
The dimension of the subspace corresponds to the size of the SDP.
%
See \pref{sec:sdp-model} for a detailed discussion of the model.

In this work, we exhibit unconditional lower bounds in
this powerful non-uniform model of computation.  For example, we show that
the \maxthreesat problem cannot be approximated to a factor better
than $7/8$ using a polynomial-size family of SDP relaxations.  Formally, we
show the following lower bound for \maxthreesat.
\begin{theorem} \label{thm:maxthreesat}
  For every $s>7/8$, there exists a constant $\alpha>0$ such that for every $n\in \N$ and every linear subspace $U$ of functions $f\from \{0,1\}^n\to \R$ with
  \begin{displaymath}
    \dim U \le n^{\alpha \frac{\log n}{\log \log n}}\mcom
  \end{displaymath}
  there exists a \maxthreesat instance $\inst$ on $n$ variables such that $\max(\inst)\le s$ but $\sosub_U(\inst)=1$ (i.e., $U$ fails to achieve a factor-$s$ approximation for \maxthreesat).
\end{theorem}

Our main result is a characterization of
an optimal semidefinite
programming relaxation for the class of constraint satisfaction
problems among all families of SDP relaxations of similar size.
%
Roughly speaking, we show that the $O(1)$-degree sum-of-squares relaxations
are {\it optimal} among all polynomial-sized SDP relaxations for constraint
satisfaction problems.
%
Towards stating our main result, we define the class of constraint
satisfaction problems.  For the sake of clarity, we restrict
ourselves to boolean constraint satisfaction problems although the
results hold in greater generality.
%
%

For a finite collection $\scrP$ of $k$-ary predicates $P\from \{0,1\}^k\to \{0,1\}$, we let \maxscrP denote the following optimization
problem:
%
An instance $\inst$ consists of boolean variables $X_1,\ldots,X_n$ and
a collection of $\scrP$-constraints $P_1(X)=1,\ldots,P_M(X)=1$ over
these variables.
%
A $\scrP$-constraint is a predicate $P_0\from \{0,1\}^n\to \{0,1\}$ such
that $P_0(X)=P(X_{i_1},\ldots,X_{i_k})$ for some $P\in\scrP$ and \emph{distinct} indices
$i_1,\ldots,i_k\in[n]$.
%
The objective is to find an assignment $x\in \{0,1\}^n$ that satisfies as
many of the constraints as possible, that is, which maximizes
\begin{displaymath}
  \inst(x)\defeq \frac{1}{M} \sum_{i=1}^M P_i(x)\mper
\end{displaymath}
%

We denote the optimal value of an assignment for $\inst$ as
$\opt(\inst)=\max_{x\in\{0,1\}^n}\inst(x)$.
For example, \maxcut corresponds to the case where $\scrP$ consists of
the binary inequality predicate.
For \maxthreesat, $\scrP$ contains all eight 3-literal disjunctions,
e.g., $X_1\vee \bar X_2\vee \bar X_3$.

%

Next, we discuss how to compare the quality of upper bound
certificates of the form $\sosub_U$.
Let $\Pi$ be a boolean CSP and let $\Pi_n$ be the restriction of $\Pi$
to instances with $n$ boolean variables.
As discussed before, the problem $\Pi_n$ could for example be \maxcut on graphs with $n$ vertices or \maxthreesat on formulas with $n$ variables.
We say that a subspace $U\subseteq \R^{\{0,1\}^n}$ achieves a \emph{$(c,s)$-approximation for $\Pi_n$} if every instance $\inst\in \Pi_n$ satisfies
\begin{equation}
\label{eq:c-s-approximation}
  \max(\inst)\le s \quad
  \Longrightarrow\quad \sosub_U(\inst)\le c \mper
\end{equation}
%
In other words, the upper bound $\sosub_U$ allows us to distinguish\footnotemark\ between the cases $\max(\inst)\le s$ and $\max(\inst)>c$ for all instances $\inst\in \Pi_n$.
\footnotetext{In order to distinguish between the cases
	$\max(\inst)\le s$ and $\max(\inst)>c$ it is enough to
	check whether $\inst$ satisfies $\sosub_U(\inst)\le c$.
In the case $\max(\inst)\le s$, we know that $\sosub_U(\inst)\le c$ by \pref{eq:c-s-approximation}.
On the other hand, in the case $\max(\inst)>c$, we know that $\sosub_U(\inst)>c$ because $\sosub_U(\inst)$ is always an upper bound on $\max(\inst)$.}

We prove the following theorem, which shows that for every
boolean CSP, the approximation guarantees obtained by the degree-$d$ sum-of-squares upper bound (also
known as the the level-$d/2$ Lasserre SDP relaxation) are optimal among all semidefinite programming relaxations of size at
most $n^{cd}$ for some universal constant $c > 0$.
\begin{theorem}\label{thm:csp-intro}
  Let $\Pi$ be boolean constraint satisfaction problem and let $\Pi_n$ be the set of instances of $\Pi$ on $n$ variables.
  Suppose that for some $m,d\in \N$, the subspace of degree-$d$ functions $f\from \{0,1\}^m\to\R$ fails to achieve a $(c,s)$-approximation for $\Pi_m$ (in the sense of \pref{eq:c-s-approximation}).
  Then there exists a number $\alpha=\alpha(\Pi_m,c,s)>0$ such that for all $n\in \N$, every subspace $U$ of functions $f\from \{0,1\}^n\to\R$ with $\dim U \le \alpha \cdot (n/\log n)^{d/4}$ fails to achieve a $(c,s)$-approximation for $\Pi_n$.
\end{theorem}

The theorem has several immediate concrete consequences for specific
boolean CSPs.  First, we know that $O(1)$-degree sos upper bounds do
not achieve an approximation ratio better than $7/8$ for \maxthreesat
\cite{Grigoriev2001, schoenebeck2008linear}, therefore \pref{thm:csp-intro}
implies that polynomial-size SDP relaxations for \maxthreesat cannot achieve an approximation ratio better than $7/8$.
In fact, a quantitatively stronger version of the above theorem yields \pref{thm:maxthreesat}.

Another concrete consequence of this theorem is that if there exists a polynomial-size family
of semidefinite programming relaxations for \maxcut that achieves an approximation ratio better than $\alpha_{\mathrm{GW}}$, then also a $O(1)$-degree sum-of-squares upper bound achieves such a ratio.
%
This assertion is especially significant in light of the notorious Unique Games
Conjecture one of whose implications is that it is NP-hard to
approximate \maxcut to a ratio strictly better than $\alpha_{GW}$.
%
%

\Jcomment{I comment the reference to the UGC.  It does not seem (to me) to follow from \pref{thm:csp-intro}.}

%
%
%
%







\Dnote{}

%
%
%
%
%

\Jnote{}
%
%




%

%

\Dnote{}
\Pnote{}





\subsection{Positive semidefinite rank and sum-of-squares degree}
\label{sec:sos-degree}

%

In order to prove our results on spectrahedral lifts and semidefinite relaxations, the
factorization perspective will be essential.
In the  LP setting, the characterization of polyhedral lifts and LP relaxations in terms of nonnegative factorizations is a significant contribution of Yannakakis \cite{Yannakakis91}.
In the SDP setting, the analogous characterization is in terms of positive semidefinite factorizations
 \cite{FMPTW12,GouveiaParriloThomas2011}.

\begin{definition}[PSD rank]
Let $M \in \mathbb R_+^{p \times q}$ be a matrix with non-negative entries.  We say that $M$ admits
a \emph{rank-$r$ psd factorization} if there exist positive semidefinite matrices $\{A_i : i \in [p]\},
\{B_j : j \in [q]\} \subseteq \cS_+^r$ such that $M_{i,j}= \Tr(A_i B_j)$ for all $i \in [p], j \in [q]$.
We define $\psdrank(M)$ to be the smallest $r$ such that $M$ admits a rank-$r$ psd factorization.
We refer to this value as the \emph{psd rank of $M$.}
\end{definition}

\Dnote{}
Nonnegative factorizations correspond to the special case that the matrices $\{A_i\}$ and $\{B_j\}$ are restricted to be diagonal.
A rank-$r$ nonnegative factorization can equivalently be viewed as a sum of $r$ rank-$1$ nonnegative factorizations (nonnegative rectangles).
Indeed, this viewpoint is crucial for all lower bounds on nonnegative factorization.
In contrast, rank-$r$ psd factorizations do not seem to admit a good characterization in terms of rank-$1$ psd factorizations.
This difference captures one of the main difficulties of proving psd rank lower bounds.

\paragraph{Main theorem}

Consider a nonnegative function $f\from \{0,1\}^n \to \R_+$ on the $n$-dimensional discrete cube.
We say that $f$ has a \emph{sum-of-squares (sos) certificate of degree $d$}
if there exist functions $g_1, \ldots, g_k\from \{0,1\}^n\to \R$
such that $\deg(g_1),\ldots,\deg(g_k) \leq d/2$, and $f(x)=\sum_{i=1}^k g_i(x)^2$
for all $x \in \{0,1\}^n$.
(Here, the $\deg(g)$ denotes the degree of $g$ as a multilinear polynomial.
We refer to Section \ref{sec:prelims} for the precise definition.)
We then define the \emph{sos degree of $f$}, denoted $\sosdeg(f)$, to be the minimal
$d$ such that $f$ has a degree-$d$ sos certificate.
%
%
%
%
%
%

This notion is closely related\footnote{For the sake of simplicity,
we have only defined this notion for functions on the discrete cube.
In more general settings, one has to be a bit more careful;
we refer to \cite{GV02}.}
 to (a special case of) the Positivstellensatz
proof system of Grigoriev and Vorobjov \cite{GV02}.
We refer to the surveys \cite{LaurentSurvey09, DBLP:journals/corr/BarakS14} and the introduction of \cite{OZ12}
for a review of such proof systems and their relationship to semidefinite programming.

With this notion in place, we can now present a representative theorem
that embodies our approach.
For a point $x \in \bbR^n$ and a subset $S \subseteq [n]$, we
denote by $x_S \in \bbR^{|S|}$ the vector $x_S = (x_{i_1}, x_{i_2}, \ldots, x_{i_{|S|}})$
where $S = \{i_1, i_2, \ldots, i_{|S|}\}$ and $i_1 < i_2 < \cdots < i_{|S|}$.
For a function $f : \{0,1\}^m \to \Rnn$ and a number $n \geq m$,
we define the following central object:
The $\binom{n}{m} \times 2^n$-dimensional real matrix $M_n^f$ is given by
\begin{equation}\label{eq:restriction}
M^f_n(S,x) \defeq f(x_S)\,,
\end{equation}
where $S \subseteq [n]$ runs over all subsets of size $m$ and $x \in \{0,1\}^n$.

\begin{theorem}[Sum-of-squares degree vs. psd rank]
\label{thm:sos-vs-psd}
For every $m \geq 1$ and $f \from \{0,1\}^m \to \Rnn$,
there exists a constant $C > 0$ such that the following holds.
%
For $n \geq 2m$,
if $d+2 = \sosdeg(f)$, then
\[
1+n^{1+ d/2} \geq \psdrank(M^f_n) \geq C \left(\frac{n}{\log n}\right)^{d/4}\,.
\]
%
\end{theorem}

\Pnote{}

\begin{remark}
The reader might observe that the matrix in \eqref{eq:restriction} looks very similar to the
``pattern matrices'' defined by Sherstov \cite{Sherstov2011}.
This comparison is not unfounded;
some high-level aspects of our proof are quite similar to his.
Random restrictions are a powerful tool for analyzing functions over the discrete cube.
We refer to \cite[Ch. 4]{OD14} for a discussion of their utility in the
context of discrete Fourier analysis.  They were also an important tool
in the work \cite{DBLP:conf/focs/ChanLRS13} on lower bounds for LPs.
Accordingly, one hopes that our methods may have additional applications in
communication complexity.
This would not be surprising, as there is a model of quantum communication
that exactly captures psd rank (see \cite{FMPTW12}).
\end{remark}

\paragraph{Connection to spectrahedral lifts of polytopes}

The connection to psd lifts proceeds as follows.
Let $\{x_1, x_2, \ldots, x_{v}\} \subseteq P$ be such that $P = \mathrm{conv}(V)$ is the convex hull of $V$, and also fix
a representation
\[
P = \left\{ \vphantom{\bigoplus} x \in \mathbb R^n : \langle a_i, x\rangle \leq b_i \,\, \forall i \in [m]\right\}\,.
\]
The \emph{slack matrix $S$} associated to $P$ (and our chosen representation) is the matrix $S \in \Rnn^{m \times v}$ given by
$S_{i,j} = b_i - \langle a_i, x_j\rangle$.   It is not difficult to see that $\psdrank(S)$ does not depend on
the choice of representation.  It turns out that the psd rank of $S$ is precisely the minimum size
of a psd lift of $P$.

\begin{proposition}[\cite{FMPTW12,GouveiaParriloThomas2011}]
\label{prop:gpt}
For every $n,k \geq 1$, every polytope $P \subseteq \mathbb R^n$ and every slack matrix $S$ associated to $P$, it
holds that $\psdrank(S) \leq k$ if and only if $P$ admits a psd lift of size $k$.
\end{proposition}


Thus our goal in this paper becomes one of proving lower bounds on psd rank.
With this notation, we have a precise way to characterize the lack of previous progress:  Before this work,
there was no reasonable method available to prove lower bounds on the psd rank of explicit matrices.
The characterization of \pref{prop:gpt}
explains our abuse of notation in
\pref{thm:corr-lb}, writing $\psdrank(P)$ to denote the psd rank
of any slack matrix associated to a polytope $P$.

\pref{thm:sos-vs-psd} is already enough to show that $\psdrank(\corr_n)$ must grow faster than
any polynomial in $n$, as we will argue momentarily.  In \pref{sec:proof-of-main-theorem}, we present a more refined version
(using a more robust version of sos degree) that will allow us to achieve a lower bound of the form $\psdrank(\corr_n) \geq 2^{\Omega(n^{\delta})}$
for some $\delta > 0$.

%
%
%
\Jnote{}

\Dnote{}


%
%
%

\Jnote{}


\Dnote{}
\Dnote{}

Given \pref{thm:sos-vs-psd}, in order to prove a lower bound on $\psdrank(\corr_n)$, we should find,
for every $d \geq 1$, a number $m$ and a function $f : \{0,1\}^m \to \Rnn$ such that $\sosdeg(f) \geq d$
and such that $M_n^f$ is a submatrix of some slack matrix associated to $\corr_n$.
To this end, it helps to observe the following (we recall the proof in Section \ref{sec:corr}).

\begin{proposition}
\label{prop:quadric-intro}
If $f \from \{0,1\}^m \to \Rnn$ is a nonnegative quadratic function over $\{0,1\}^m$,
then for any $n \geq m$, the matrix $M_n^f$ is a submatrix of some slack matrix associated to $\corr_n$.
\end{proposition}

\begin{comment}
The correlation polytope is also referred to as the \emph{Boolean quadric polytope} \cite{Padberg89} for
the following reason.
Suppose that $\ell_{y,a}(x) = a-\sum_{i=1}^n y_i x_i$ is a linear
form in the variables $\{x_i\}$.
If, for some $a, b \in \mathbb R$ and $y \in \mathbb R^n$, we have
\[
\ell_{y,a}(x)^2 \geq b\qquad \forall x \in \{0,1\}^n,
\]
then there is a corresponding valid linear inequality for $\corr_n$ in the sense that,
for $x \in \{0,1\}^n$,
\begin{equation}\label{eq:corr-ineq}
b \leq \ell_{y,a}(x)^2 = (a - y^T x)^2 = a^2 + (y^T x)^2 - 2 a y^T x = a^2 + \langle yy^T, xx^T\rangle - 2 a \langle \mathrm{diag}(y), xx^T\rangle\,,
\end{equation}
where we have used the notation $\mathrm{diag}(y)$ for the diagonal matrix with the entries of $y$ on the diagonal, and
$\langle A,B\rangle = \Tr(A^T B)$ denotes the Frobenius inner product.
Note our use of the fact that $\langle \mathrm{diag}(y), \mathrm{diag}(x)\rangle = \langle \mathrm{diag}(y), xx^T\rangle$
which is true for $x \in \{0,1\}^n$.

If \eqref{eq:corr-ineq} holds for all $x \in \{0,1\}^n$, then by convexity we have, for every $Z \in \corr_n$,
\[
a^2 + \langle yy^T, Z\rangle - 2 a \langle \mathrm{diag}(y), Z\rangle - b\geq 0\,.
\]


Thus if $f : \{0,1\}^m \to \Rnn$ is given by $f(x)=(a-\sum_{i=1}^m x_i)^2-b$, then $M_n^f$ is a submatrix
of some slack matrix associated to $\corr_n$ since
\[
M_n^f(S,x) = f(x_S) = \ell_{\1_S,a}(x)^2-b\,,
\]
where $\1_S$ is the indicator vector with ones in the positions corresponding to $S$.
\end{comment}

Given the preceding proposition, the following result of Grigoriev on the Knapsack tautologies
completes our quest for a lower bound.
\begin{theorem}[\cite{DBLP:journals/cc/Grigoriev01}]
\label{thm:grigor}
For every odd integer $m \geq 1$,
the function $f : \{0,1\}^m \to \Rnn$ given by
\begin{equation}\label{eq:knapsack}
f(x) = \left(\frac{m}{2}-\sum_{i=1}^m x_i\right)^2 - \frac14
\end{equation}
has $\sosdeg(f) \geq m+1$.
\end{theorem}

Note that since $m/2$ is not an integer, \eqref{eq:knapsack}
is nonnegative for all $x \in \{0,1\}^m$.
It turns out that in order to prove stronger lower bounds for $\corr_n$,
we will require a lower bound on the \emph{approximate} sos degree of $f$.
Thus the Knapsack tautologies \eqref{eq:knapsack} will be studied carefully
in \pref{sec:psd-corr}.
In \pref{sec:overview}, we discuss the proof of \pref{thm:sos-vs-psd}
in some detail.  Then in \pref{sec:theproof}, we present a quantitatively
stronger theorem and its proof.
%


\paragraph{Connection to semidefinite relaxations and constraint satisfaction}

Fix now numbers $k,n \geq 1$ and a boolean CSP $\Pi$.  Fix a
pair of constants $0 \leq s \leq c \leq 1$.  Suppose our goal is to
show a lower bound on the size of SDP relaxations that yield a
$(c,s)$-approximation on instances of size $n$.
%
It turns out that this task reduces to proving a lower bound on the
positive semidefinite rank of an explicit matrix $M$ indexed by problem instances and problem solutions (points on the discrete cube in our case).
%
\begin{proposition}
\label{prop:intro-csp2}
  For any boolean CSP $\Pi_n$ and any constants $0 \leq s<c \leq 1$, let $U$ be a subspace of minimal dimension that achieves a $(c,s)$-approximation for $\Pi_n$.
  Denote the set of instances
  \[\Pi_n^{\le s}=\{\inst \mid \max(\inst)\le s\}\,.\]
  Let $M\from \Pi_n^{\le s}\times \{0,1\}^n\to \R$ denote the matrix
  \begin{displaymath}
    M(\inst, x ) = c - \inst(x)\mper
  \end{displaymath}
  Then, $ \psdrank(M)^2\geq \dim(U) \geq \psdrank(M)$.
\end{proposition}

Before describing the proof of this proposition, observe that together with our main theorem the proposition implies \pref{thm:csp-intro} (optimality of degree-$d$ sum-of-squares for approximating boolean CSPs):
If $\inst_0$ is a \maxscrP instance on $m$ variables with $\max(\inst_0)\le s$ and $\sosub_d(\inst_0)>c$, then $f=c-\inst_0$ has sos degree larger than $d$.
Our main theorem gives a lower bound on the psd rank of the matrix $M^f_n$.
Since this matrix is a submatrix of the matrix in \pref{prop:intro-csp2}, our psd rank lower bound implies a lower bound on the minimum dimension of a subspace achieving a $(c,s)$-approximation for $\maxscrP_n$.

%
%
\begin{proof}[Proof of \pref{prop:intro-csp2}]
Set $r = \dim(U)$.  Fix a basis $q_1,\ldots, q_r : \bits^n \to \R$
for the subspace $U$.  Define the function $Q : \bits^n \to \cS_r^+$
by setting $(Q(x))_{ij} \seteq q_i(x) q_j(x)$ for all $i,j \in [r]$.
Notice that for any $q \in U$, we can write $q = \sum_{i=1}^r \lambda_i q_i$
and thus $q(x)^2 = \Tr(\Lambda Q(x))$ where $\Lambda \in \cS_r^+$ is
defined by $\Lambda_{ij} \seteq \lambda_i \lambda_j$.

Since $U$ achieves a $(c,s)$-approximation for $\Pi_n$, for every
instance $\inst \in \Pi_n^{\leq s}$ we will have
$\sosub_{U}(\inst) \leq c$.  By definition of
$\sosub_{U}(\inst)$, this implies that $c - \inst = \sum_i
g_i^2$ for $g_i \in U$.  By expressing each $g_i^2$ as $g_i^2 =
\Tr(\Lambda_i Q(x))$
for some $\Lambda_i \in \cS_r^+$ we get,
$$ M(\inst, x) = c - \inst(x) = \sum_i \Tr(\Lambda_i Q(x)) = \Tr\left(
\Lambda_{\inst} Q(x)\right) \mper$$
This yields an explicit psd factorization of $M$ certifying that
$\psdrank(M) \leq \dim(U)$.

Conversely, by definition of $\psdrank(M)$ there exists positive
semidefinite matrices $\{\Lambda_{\inst} : \inst \in \Pi_n^{\leq s}\}$, $\{ Q(x) : x \in \bits^n \} \sse \cS_r^+$ such that $M(\inst,x) =
\Tr(\Lambda_{\inst} Q(x))$.  Denote by $R(x) \seteq Q(x)^{1/2}$
the positive semidefinite square root, and consider
the subspace $\tilde{U}
\seteq \mathrm{span}\{ (R(x))_{ij} \} \sse \R^{\bits^n}$.  Clearly,
the dimension of $\tilde{U}$ is at most $\psdrank(M)^2$.  Further, for each instance
$\inst \in \Pi_n^{\leq s}$, we can write
$$ c - \inst = M_{\inst, x} = \Tr(\Lambda_{\inst} Q(x)) =
\Tr(\Lambda_{\inst} R(x)^2) = \norm{\sqrt{\Lambda_\inst} R(x)}_F^2
\mper$$
Observe that $\norm{\sqrt{\Lambda_{\inst}}R(x)}_F^2$ is a sum of
squares of functions from the subspace $\tilde{U}$\footnote{Here,$\|\cdot\|_F$ denotes
the Frobenius norm.}.  Therefore we have
$\sosub_{\tilde{U}}(\inst) \leq c$, showing that $\sosub_{\tilde{U}}$ yields a
$(c,s)$-approximation to $\Pi_n$.  Since $U$ is the minimal subspace
yielding a $(c,s)$-approximation, we have $\dim(U) \leq
\dim(\tilde{U}) \leq \psdrank(M)^2$.
\end{proof}








\begin{comment}

For $0 \leq s \leq c \leq 1$, we define the matrix (represented in
the form of a function for convenience of notation):
\[
M^{n,\Pi}_{c,s}(\inst, x) \defeq c - \inst(x)\,,
\]
where the first index of $M^{n,\Pi}_{c,s}$ ranges over all instances on $n$ variables satisfying $\opt(\inst) \leq s$.
A ``certificate'' that this matrix is nonnegative corresponds to the ability to prove that $\opt(\inst) \leq c$
whenever $\opt(\inst) \leq s$.  The connection to approximation should be readily apparent.
We provide a way to prove a lower bound on the psd rank of such matrices;
this corresponds to proving hardness of approximation in the SDP framework.
The method is via an intimate relationship to sos degree; we provide
a restatement of \pref{thm:sos-vs-psd} in this setting.



\Jnote{}

The point now is that the matrix $M_n^f$ in the preceding theorem
occurs as a submatrix of $M^{n,\Pi}_{c,s}$.
Using known lower bounds on sos degree (see, for instance, \cite{Grigoriev2001} and \cite{schoenebeck2008linear}),
one obtains results like the following.
\end{comment}

\begin{comment}

\subsection{Statement of results}
\label{sec:results}

We now state the main consequences of our psd rank lower bounds.


\paragraph{Approximation complexity of max-CSPs}
In \pref{sec:maxcsp}, we state explicitly our model
of approximation for SDPs.
But it is possible to state the results equivalently in the language of psd rank, and we do so now.


\Dnote{}

\begin{theorem}
\label{thm:sos-vs-sdp-csps}
For every $0 \leq s \leq c \leq 1$, the following holds.
Consider some $m \geq 1$ and an instance $\inst$ of \maxscrP with $\opt(\inst) \leq s$.
Define $f : \{0,1\}^m \to \Rnn$ by $f(x) = c - \inst(x)$.  If $d = \sosdeg(f)$, then
there exists a constant $C > 0$ such that
for every $n \geq 2m$,
\[
\psdrank(M_n^f) \geq C \left(\frac{n}{\log n}\right)^{d/4}\,.
\]
\end{theorem}


%

\begin{theorem} \label{thm:maxthreesat}
Let $\scrP$ be the set of predicates corresponding to \maxthreesat.  Then for any $s > 7/8$ and any $n \geq 1$, we have
\[
\psdrank(M^{n,\scrP}_{1,s}) \geq n^{\Omega(\frac{\log n}{\log \log n})}\,.
\]
\end{theorem}
This implies that no family of polynomial-size SDPs for \maxthreesat can have an integrality gap better than $7/8$;
see \pref{sec:maxcsp}.

\end{comment}

\begin{comment}
Fix a finite set $\Omega$, and let $\cF$ be a family of nonnegative functions $f\from \Omega \to \R_+$.
One might think of $\Omega$ as the $n$-dimensional discrete cube $\{-1,1\}^n$, the set of perfect matchings on $2n$ vertices,
or the set of tours on $n$ cities.
We ask if there exists a ``compact way'' to certify nonnegativity of all the functions in the family $\cF$.


Let $B\from \Omega \to \R^{r \times r}$ be a matrix-valued function on $\Omega$.
We say that $B$ is a \emph{rank-$r$ certificate for nonnegativity of $\cF$} if every function $f \in \cF$ can be written as
\[
f(x) = \|A \cdot B(x)\|_F^2
\]
for some matrix $A \in \bbR^{r \times r}$.  Here, we use $\|\cdot\|_F$ to denote the Frobenius norm of a matrix.
Consider now the matrix $M \in \R_+^{\cF \times \Omega}$ with $M(f,x)=f(x)$.

\begin{lemma}
For any such $M$, $\psdrank(M)$ is precisely the smallest value $r$ such that
$\cF$ admits a rank-$r$ certificate for nonnegativity.
\end{lemma}

Given the preceding lemma, we will allow ourselves to abuse notation by writing $\psdrank(\cF)$.
For simplicity, let us now fix $\Omega = \{-1,1\}^n$.
For a nonnegative function $f : \{-1,1\}^n \to \mathbb R_+$, we define the \emph{sos-degree of $f$}
as the smallest $d$ such that $f(x) = p(x)^2$, where $\deg(p(x)^2) \leq d$ when $p$ is considered
as a polynomial over the discrete cube.
\end{comment}

%
%
%
%

==> preamble/macros-sdpsize.tex <==

% abbreviations and paper-specific macros

\let\pref=\prettyref

\renewcommand{\Vsymb}{\mathrm{Var}}

\newcommand*{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

% \setlength{\parskip}{2pt}

\let\super\varsuper
\newcommand*{\id}{\mathrm{id}}

\newcommand*{\qe}[2]{S(#1\,\|\, #2)}
\newcommand*{\ce}[2]{D(#1\,\|\, #2)}

\newcommand*{\sst}{\substack}
\renewcommand{\Ind}{\bm 1}
\ifnum\jamesmode=0
% \renewcommand{\Ind}{\vvmathbb 1}
\fi
\let\1\Ind

\newcommand*{\hi}{\mathsf{high}}
\newcommand*{\low}{\mathsf{low}}

\newcommand*{\inst}{\Im}
\newcommand*{\GF}[1]{\mathbb F_{#1}}

\newcommand*{\gtwo}{\gamma_{2\to 2}^{\mathsf{psd}}}
\newcommand*{\psdrank}{\mathrm{rk}_{\mathsf{psd}}}
\newcommand*{\apsdrank}{\rho_{\mathsf{psd}}}
\newcommand*{\nnrank}{\mathrm{rk}_{+}}
\newcommand*{\sosdeg}{\deg_{\mathsf{sos}}}
\newcommand*{\juntadeg}{\deg_{\mathsf{J}}}

\newcommand{\polytope}[1]{\text{\textup{\textsc{#1}}}}

\newcommand*{\corr}{\polytope{corr}}
\newcommand*{\tsp}{\polytope{tsp}}
\newcommand*{\cut}{\polytope{cut}}
\newcommand*{\stab}{\polytope{stab}}

\newcommand*{\ot}{\otimes}
\newcommand*{\pmo}{\{\pm 1\}}


\newcommand*{\maxpi}{\problemmacro{max-$\Pi$}}
\newcommand*{\maxscrP}{\problemmacro{max-$\scrP$}}
\newcommand*{\maxthreecnf}{\problemmacro{max \pnum{3}-cnf}}


% \newcommand*{\pE}{\tilde {\mathbb E}}

\newcommand*{\sleq}{\preceq}
\newcommand*{\sgeq}{\succeq}

\DeclareMathOperator{\Id}{\mathrm{Id}}

\DeclareMathOperator{\pE}{\tilde {\mathbb E}}

% uniform density operator

% \newcommand*{\uId}{\tfrac 1 {\Tr \Id}\Id}
\newcommand*{\uId}{\mathcal{U}}

\newcommand*{\annotaterel}[2]{\stackrel{\scriptscriptstyle\text{#1}}{#2}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../sdpsize"
%%% End:

